Can decaying dark matter scenarios alleviate both $H_0$ and $\sigma_8$ tensions?

Current tensions in cosmology, including $H_0$ and $\sigma_8$, provide one of the strong reasons to suspect the existence of physics beyond the standard model of cosmology ($\Lambda$CDM). In this paper, we investigate if there is a relation between these tensions and beyond cold dark matter scenarios. To model non-CDM, we assume a decaying dark matter (DDM) which is unstable and may decay into two daughter particles, a combination of cold dark matter, warm dark matter, and dark radiation, to explore a vast era of possibilities. We checked our model against CMB data and could show that decaying dark matter seems not a promising candidate to address the cosmological tensions.

==> document.tex <==
\Omega_B = 0.04864\pm 0.00059
\Omega_B = 0.0486^{+0.0011}_{-0.0012}
\Omega_B = 0.0486^{+0.0015}_{-0.0015}
\Omega_{DM} = 0.2567\pm 0.0066
\Omega_{DM} = 0.257^{+0.012}_{-0.013}
\Omega_{DM} = 0.257^{+0.017}_{-0.017}
100\theta_s = 1.04194\pm 0.00029
100\theta_s = 1.04194^{+0.00060}_{-0.00055}
100\theta_s = 1.04194^{+0.00076}_{-0.00076}
ln10^{10}A_s = 3.058^{+0.013}_{-0.015}
ln10^{10}A_s = 3.058^{+0.029}_{-0.028}
ln10^{10}A_s = 3.058^{+0.039}_{-0.040}
n_s = 0.9726^{+0.0037}_{-0.0043}
n_s = 0.9726^{+0.0082}_{-0.0078}
n_s = 0.973^{+0.011}_{-0.010}
\tau_{reio} = 0.0595^{+0.0067}_{-0.0080}
\tau_{reio} = 0.059^{+0.016}_{-0.014}
\tau_{reio} = 0.059^{+0.020}_{-0.019}
H_0 = 68.00\pm 0.54
H_0 = 68.0^{+1.1}_{-1.0}
H_0 = 68.0^{+1.4}_{-1.4}
\sigma_8 = 0.8133\pm 0.0061
\sigma_8 = 0.813^{+0.012}_{-0.012}
\sigma_8 = 0.813^{+0.015}_{-0.017}

